Exceptional Mechanical Performance by Spatial Printing with Continuous Fiber: Curved Slicing, Toolpath Generation and Physical Verification

This work explores a spatial printing method to fabricate continuous fiber-reinforced thermoplastic composites (CFRTPCs), which can achieve exceptional mechanical performance. For models giving complex 3D stress distribution under loads, typical planar-layer based fiber placement usually fails to provide sufficient reinforcement due to their orientations being constrained to planes. The effectiveness of fiber reinforcement could be maximized by using multi-axis additive manufacturing (MAAM) to better control the orientation of continuous fibers in 3D-printed composites. Here, we propose a computational approach to generate 3D toolpaths that satisfy two major reinforcement objectives: 1) following the maximal stress directions in critical regions and 2) connecting multiple load-bearing regions by continuous fibers. Principal stress lines are first extracted in an input solid model to identify critical regions. Curved layers aligned with maximal stresses in these critical regions are generated by computing an optimized scalar field and extracting its iso-surfaces. Then, topological analysis and operations are applied to each curved layer to generate a computational domain that preserves fiber continuity between load-bearing regions. Lastly, continuous fiber toolpaths aligned with maximal stresses are generated on each surface layer by computing an optimized scalar field and extracting its iso-curves. A hardware system with dual robotic arms is employed to conduct the physical MAAM tasks depositing polymer or fiber reinforced polymer composite materials by applying a force normal to the extrusion plane to aid consolidation. When comparing to planar-layer based printing results in tension, up to 644% failure load and 240% stiffness are observed on shapes fabricated by our spatial printing method.

==> text/relatedWork.tex <==
\section{Related Work}~\label{Sec:RelatedWork}
In this section, we review the most recent research in 3D printing of continuous fiber-reinforced composites, as well as the related works on multi-axis 3D printing.

\subsection{Additive Manufacturing with CFRTPCs}
Fabricating high-performance CFRTPCs through additive manufacturing has caught significant research attention over the past decade~\cite{kabir2020critical}. Two major processes, in-nozzle impregnation~\cite{Matsuzaki2016_SciReport} and out-of-nozzle impregnation~\cite{DICKSON2017146}, have been developed to infuse continuous fibers with matrix materials and create tight bonding. Efforts to optimize the performance of CFRTPCs have been examined from different perspectives -- for example, optimizing printing parameters such as temperature and layer height~\cite{Tian16_composite, heidari2019mechanical} and developing post-processing techniques~\cite{Omuro2017, Nekoda21_AdditManu}. Companies such as MarkForged~\cite{Eiger}, Anisoprint~\cite{Anisoprint}, and 9T Lab~\cite{9TLab} have also developed commercially available 3D printers that aim at massive production of CFRTPCs using additive manufacturing.

The anisotropic properties of the continuous fiber have been considered in~\cite{heitkamp2023stress, Sugiyama20_CST, Narasimha20_SciReport} to design optimized toolpaths for improving the mechanical performance of CFRTPCs. As maximal tensile strength can be observed along the axial direction of fibers, existing works usually attempt to generate stress-aligned toolpaths. A pioneering study conducted by Li~\textit{et al.}~\cite{Li2020_CompositeB} demonstrated the effectiveness of aligning continuous fibers with stress directions, achieving a remarkable increase in mechanical strength while using the same amount of fiber content. Similar results were also reported in our previous work~\cite{chen2022field}, where both the direction and density of fiber placement were controlled based on stress distribution. Moreover, integrating topology optimization into the workflow has yielded compelling results, showcasing improvements in the weight-to-strength ratio of fabricated components~\cite{Li2020_CompositeB, Ting21_CompositesA}. A recent work by Liu \textit{et al.}\cite{liu2023stress} demonstrated the ability to design toolpaths for continuous fibers using principal stress lines as guidance~\cite{Eder21_JMP}, which leads to optimized composite performance. While most existing methods focus on toolpath design for planar layers, extending them to curved layers inside solids with complex shapes is challenging (ref.~\cite{fang2020reinforced,zhang2022s3}). In this paper, we introduce a field-based approach for generating spatial fiber toolpaths that achieve stress alignment and enhanced continuity in 3D, which together result in exceptional mechanical performance of CFRTPCs made by MAAM.


\subsection{Spatial Toolpath Generation}
By higher degrees-of-freedom motion enabled using robotic arms~\cite{urhal2019robot} or CNC machines~\cite{zhang2021singularity}, MAAM hardware allows a printer head to dynamically change its orientation for aligning materials in 3D~\cite{chakraborty2008extruder}. This technology has been employed to facilitate advanced printing objectives including support-free~\cite{dai2018support}, improved surface quality~\cite{etienne2019curvislicer}, and controlled  anisotropy of materials~\cite{fang2020reinforced}. Research efforts have been made to print different materials with a MAAM system, including polymers~\cite{huang2021conformal}, composites~\cite{zhang2023robot}, metals~\cite{bhatt2022robot}, and conductive filaments~\cite{hong20235}, where different design objectives are considered. 

To fully utilize the capabilities of a MAAM system, the method for generating effective spatial toolpaths plays a critical role. Existing methods typically first decompose a solid model into curved layers, and then generate curved toolpaths on those curved surfaces~\cite{fang2020reinforced, xu2019curved, bi2023strength}. Specifically, Dai \textit{et al.}~\cite{dai2018support} introduced a method based on voxel-growing that can produce support-free printing sequences for polymer printing. Layer-free methods that directly generate printing toolpaths by decomposing the 3D design space have also been presented in~\cite{cam2023fluid, retsin2016discrete}. When printing materials with high anisotropy, Guidetti~\textit{et al.}~\cite{guidetti2023stress} designed the MAAM toolpath for liquid crystal polymers, achieving a $20\times$ higher breaking force. Toolpaths that are conformally printed on curved surfaces with continuous carbon fiber using the setup with a robotic arm have been reported in~\cite{zhang2023robot, shembekar2019generating}. However, none of these works have addressed the challenge of 3D layer generation and spatial toolpath computation for CFRPTCs with the objectives of following stress-flow~\cite{chen2022field} and ensuring fiber continuity~\cite{huang2023turning}. In this paper, we introduce a field-based computational pipeline to tackle this challenge of spatial toolpath generation for effective reinforcement on CFRPTCs.

% Multi-axis printing refers to the ability of a 3D printer to move along multiple axes, enabling the printing of complex, three-dimensional structures. This technology has received growing attention in recent years due to its potential to produce high-performance structures with improved mechanical properties. Multi-axis printing allows for advanced functionality in material accumulation for thermoplastic, metal, and composite printing. In particular, support-free printing, surface quality enhancement, and control of the anisotropy in materials have been widely studied. The computation of functional toolpaths for multi-axis printing is a critical aspect of this technology. A robotic system or multi-axis CNC machine has been introduced to the multi-axis printing process, which enables the material to be accumulated in 3D space.

% Toolpath planning is a crucial aspect of multi-axis printing, as it determines the sequence in which the material is deposited and the orientation of the fibers in the printed structure. Although layer-free methods have been reported, the existing methods still follow the strategy of first subtracting a volume design space into curved layers and then computing the printing toolpath on it. We also follow this strategy. In the aspect of curved layer decomposition, methods have been reported including [13], which proposes a curve-layer decomposition algorithm based on the marching cubes method, and [14], which introduces a surface-based approach for curved layer decomposition. The computation of functional toolpaths for multi-axis printing is a critical aspect of this technology. A number of studies have focused on the development of algorithms for generating optimized toolpaths for multi-axis printing, including field-based pipelines [11] and machine learning approaches [12]. Reference [15] proposes a method for generating toolpaths on curved surfaces using a combination of geometric algorithms and numerical optimization. These studies demonstrate the importance of considering both the material properties and the toolpath design in optimizing the performance of multi-axis printed structures. There is no existing work that can compute toolpaths for CFRPTs that take the material property into account. In this work, we have built a computational pipeline that follows the direction of the principal stress line and guarantees the continuity of the CCF to reach the highest strength. In particular, the critical region around the hole connection region is protected. The use of multi-axis printing and advanced toolpath planning has the potential to overcome the limitations of planar layer-based printing and produce high-performance structures with improved mechanical properties.

    
